RefineRAG: Word-Level Poisoning Attacks via Retriever-Guided Text Refinement

Retrieval-Augmented Generation (RAG) significantly enhances Large Language Models (LLMs), but simultaneously exposes a critical vulnerability to knowledge poisoning attacks. Existing attack methods like PoisonedRAG remain detectable due to coarse-grained separate-and-concatenate strategies. To bridge this gap, we propose RefineRAG, a novel framework that treats poisoning as a holistic word-level refinement problem. It operates in two stages: Macro Generation produces toxic seeds guaranteed to induce target answers, while Micro Refinement employs a retriever-in-the-loop optimization to maximize retrieval priority without compromising naturalness. Evaluations on NQ and MSMARCO demonstrate that RefineRAG achieves state-of-the-art effectiveness, securing a 90% Attack Success Rate on NQ, while registering the lowest grammar errors and repetition rates among all baselines. Crucially, our proxy-optimized attacks successfully transfer to black-box victim systems, highlighting a severe practical threat.

==> tables/table1.tex <==
\begin{table*}[t!]
\centering
\caption{Comparison of different attack methods on NQ and MS MARCO datasets.}
\label{tab:attack_comparison}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccccc}
\toprule
\multirow{3}{*}{\textbf{Attack Method}} 
    & \multicolumn{7}{c}{\textbf{NQ}} 
    & \multicolumn{7}{c}{\textbf{MS MARCO}} \\
    \cmidrule(lr){2-8} \cmidrule(lr){9-15}
    & \multirow{3}{*}[1.5ex]{\textbf{F1-score$\uparrow$}} 
    & \multicolumn{2}{c}{\textbf{ASR $\uparrow$}} 
    & \multirow{3}{*}[1.5ex]{\textbf{PPL $\downarrow$}} 
    & \multirow{3}{*}[1.5ex]{\textbf{RR $\downarrow$}} 
    & \multirow{3}{*}[1.5ex]{\textbf{GE $\downarrow$}} 
    & \multirow{3}{*}[1.5ex]{\textbf{RL}}
    & \multirow{3}{*}[1.5ex]{\textbf{F1-score$\uparrow$}} 
    & \multicolumn{2}{c}{\textbf{ASR$\uparrow$}} 
    & \multirow{3}{*}[1.5ex]{\textbf{PPL $\downarrow$}} 
    & \multirow{3}{*}[1.5ex]{\textbf{RR $\downarrow$}} 
    & \multirow{3}{*}[1.5ex]{\textbf{GE $\downarrow$}} 
    & \multirow{3}{*}[1.5ex]{\textbf{RL}} \\
    \cmidrule(lr){3-4} \cmidrule(lr){10-11}
    & & \textbf{Llama} & \textbf{Vicuna} & & & & 
    & & \textbf{Llama} & \textbf{Vicuna} & & & & \\
\midrule
PoisonedRAG (B) & \underline{0.94} & 0.54 & 0.61 & \textbf{55.11} & 0.28 & 2.21 & 1.00 & \underline{0.87} & 0.60 & \underline{0.67} & \textbf{55.88} & 0.28 & 2.21 & 1.00 \\
PoisonedRAG (W) & \textbf{0.95} & 0.59 & 0.65 & 372.93 & \textbf{0.00} & 6.54 & 0.66 & \textbf{0.95} & \underline{0.63} & 0.66 & 257.54 & \textbf{0.00} & 6.02 & 0.65 \\
Prompt Injection Attack & 0.75 & \underline{0.80} & \underline{0.75} & \underline{107.01} & 1.00 & \underline{0.88} & 1.00 & 0.77 & \textbf{0.83} & \textbf{0.81} & 137.86 & 1.00 & \underline{0.99} & 1.00 \\
Corpus Poisoning Attack & 0.66 & 0.00 & 0.00 & 8209.98 & 1.00 & 9.11 & 0.36 & 0.51 & 0.00 & 0.00 & 8247.50 & 1.00 & 9.16 & 0.29 \\
\textbf{RefineRAG} & 0.89 &  \textbf{0.90} & \textbf{0.85} & 118.33 & \underline{0.01} & \textbf{0.66} & 0.55 & 0.70 & \textbf{0.83} & \textbf{0.81} & \underline{127.53} & \underline{0.01} & \textbf{0.86} & 0.53 \\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/table10.tex <==
\begin{table}[t!]
    \centering
    \caption{Impact of Beam Size $B$ in Stage II}
    \label{tab:refinerag_beam_size}
    \begin{tabular}{c c c cc}
        \toprule
        \multirow{2}{*}{\textbf{Dataset}} &
        \multirow{2}{*}{\textbf{$B$}} &
        \multirow{2}{*}{\textbf{F1-score$\uparrow$}} &
        \multicolumn{2}{c}{\textbf{ASR$\uparrow$}} \\
        \cmidrule(lr){4-5}
        & & & \textbf{Llama} & \textbf{Vicuna} \\
        \midrule
        \multirow{3}{*}{\textbf{NQ}} 
            & 1 & 0.86 & 0.87 & 0.84 \\
            & 3 & \textbf{0.89} & \textbf{0.90} & 0.85 \\
            & 5 & 0.88 & 0.88 & \textbf{0.89} \\
        \midrule
        \multirow{3}{*}{\textbf{MSMARCO}} 
            & 1 & 0.68 & 0.77 & 0.80 \\
            & 3 & 0.70 & \textbf{0.83} & \textbf{0.81} \\
            & 5 & \textbf{0.71} & 0.79 & 0.80 \\
        \bottomrule
    \end{tabular}
\end{table}

==> tables/table3.tex <==
\begin{table*}[t!]
  \centering
  \caption{Impact of Victim Models}
  \label{tab:impact-of-llms}
  \begin{tabular}{cccc}
    \toprule
    \multirow{2}{*}{\textbf{LLM}} & \multicolumn{2}{c}{\textbf{ASR$\uparrow$}} \\ 
    \cmidrule(lr){2-3}
     & \textbf{NQ} & \textbf{MSMARCO} \\
    \midrule
    Llama2-7B     & 0.90 & 0.83 \\
    Vicuna-7B     & 0.85 & 0.81 \\
    DeepSeek-R1   & 0.84 & 0.75 \\
    DeepSeek-V3   & 0.92 & 0.78 \\
    Qwen2.5-7B    & 0.86 & 0.76 \\
    Qwen3-Max     & 0.81 & 0.73 \\
    \bottomrule
  \end{tabular}
\end{table*}

==> tables/table4.tex <==
\begin{table*}[t!]
    \centering
    \caption{Impact of Retriever.} 
    \label{tab:impact-retriever-llm}
    \begin{tabular}{c c c cc}
        \toprule
        \multirow{2}{*}{\textbf{Dataset}} & 
        \multirow{2}{*}{\textbf{Retriever}} & 
        \multirow{2}{*}{\textbf{F1-score$\uparrow$}} & 
        \multicolumn{2}{c}{\textbf{ASR$\uparrow$}} \\ 
        \cmidrule(lr){4-5}
         & & & \textbf{Llama} & \textbf{Vicuna} \\
        \midrule
        \multirow{3}{*}{\textbf{NQ}} 
            & Contriever & 0.89 & 0.90 & 0.85 \\
            & Contriever-ms & 0.79 & 0.82 & 0.80 \\
            & ANCE & 0.63 & 0.70 & 0.68 \\
        \midrule
        \multirow{3}{*}{\textbf{MSMARCO}} 
            & Contriever & 0.70 & 0.83 & 0.81 \\
            & Contriever-ms & 0.60 & 0.64 & 0.66 \\
            & ANCE & 0.47 & 0.56 & 0.60 \\
        \bottomrule
    \end{tabular}
\end{table*}

==> tables/table5.tex <==
\begin{table}[t!]
    \centering
    \caption{Ablation results of RefineRAG.}
    \label{tab:ablation_study_components}
    
    \begin{tabular}{cccc c}
        \toprule
        \multirow{2}{*}{\textbf{Dataset}} & 
        \multirow{2}{*}{\textbf{Attack}} & 
        \multirow{2}{*}{\textbf{F1-score$\uparrow$}} & 
        \multicolumn{2}{c}{\textbf{ASR$\uparrow$}} \\ 
        \cmidrule(lr){4-5}
         & & & \textbf{Llama2} & \textbf{Vicuna} \\
        \midrule
        
        \multirow{3}{*}{\textbf{NQ}}
        & \textbf{RefineRAG} & \textbf{0.89} & \textbf{0.90} & \textbf{0.85} \\
        & w/o Stage I  & 0.63 & 0.72 & 0.69 \\
        & w/o Stage II  & 0.73 & 0.86 & 0.82 \\
        \midrule

        \multirow{3}{*}{\textbf{MSMARCO}}
        & \textbf{RefineRAG} & \textbf{0.70} & \textbf{0.83} & \textbf{0.81} \\
        & w/o Stage I  & 0.53 & 0.71 & 0.75 \\
        & w/o Stage II  & 0.54 & 0.75 & 0.79 \\
        \bottomrule
    \end{tabular}
\end{table}

==> tables/table6.tex <==
\begin{table}[t!]
\centering
\caption{Impact of attacker LLMs.}
\label{tab:attacker_llm}
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & 
\multirow{2}{*}{\textbf{Generator}} & 
\multirow{2}{*}{\textbf{F1-Score$\uparrow$}} & 
\multicolumn{2}{c}{\textbf{ASR$\uparrow$}} \\ 
\cmidrule(lr){4-5}
 & & & \textbf{Llama} & \textbf{Vicuna} \\
\midrule
\multirow{2}{*}{\textbf{NQ}} 
 & DeepSeek-V3 & 0.89 & 0.90 & 0.85 \\
 & Qwen3-Max & 0.91 & 0.85 & 0.82 \\
\midrule
\multirow{2}{*}{\textbf{MSMARCO}} 
 & DeepSeek-V3 & 0.70 & 0.83 & 0.81 \\
 & Qwen3-Max & 0.74 & 0.83 & 0.83 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/table7.tex <==
\begin{table}[t!]
    \centering
    \caption{Impact of Stage I Iteration Rounds}
    \label{tab:refinerag_rounds}
    \begin{tabular}{ccccc}
        \toprule
        \multirow{2}{*}{\textbf{Dataset}} & 
        \multirow{2}{*}{\textbf{Rounds}} & 
        \multirow{2}{*}{\textbf{F1-score$\uparrow$}} & 
        \multicolumn{2}{c}{\textbf{ASR$\uparrow$}} \\ 
        \cmidrule(lr){4-5}
        & & & \textbf{Llama} & \textbf{Vicuna} \\
        \midrule
        \multirow{3}{*}{\textbf{NQ}} 
            & 3 & 0.84 & 0.84 & 0.79 \\
            & 4 & \textbf{0.89} & \textbf{0.90} & \textbf{0.85} \\
            & 5 & 0.88 & 0.86 & 0.83 \\
        \midrule
        \multirow{3}{*}{\textbf{MSMARCO}} 
            & 3 & 0.63 & 0.72 & 0.73 \\
            & 4 & \textbf{0.70} & \textbf{0.83} & \textbf{0.81} \\
            & 5 & 0.67 & 0.79 & 0.72 \\
        \bottomrule
    \end{tabular}
\end{table}

==> tables/table8.tex <==
\begin{table}[t!]
\centering
\caption{Impact of Iterations in Stage II}
\label{tab:refinerag_maxiter_sensitivity}
\begin{tabular}{c c c c c}
\toprule
\multirow{2}{*}{\textbf{Dataset}} &
\multirow{2}{*}{\textbf{Iterations}} &
\multirow{2}{*}{\textbf{F1-score$\uparrow$}} &
\multicolumn{2}{c}{\textbf{ASR$\uparrow$}} \\
\cmidrule(lr){4-5}
& & & \textbf{Llama} & \textbf{Vicuna} \\
\midrule
\multirow{3}{*}{\textbf{NQ}} 
 & 5  & 0.85 & \textbf{0.91} & \textbf{0.87}\\
 & 10 & \textbf{0.89} & 0.90 & 0.85\\
 & 15 & \textbf{0.89} & 0.88 & 0.84\\
\midrule
\multirow{3}{*}{\textbf{MSMARCO}} 
 & 5  & 0.65 & 0.79 & 0.80\\
 & 10 & 0.70 & \textbf{0.83} & \textbf{0.81}\\
 & 15 & \textbf{0.74} & 0.81 & 0.79\\
\bottomrule
\end{tabular}
\end{table}

==> tables/table9.tex <==
\begin{table}[t!]
    \centering
    \caption{Impact of Top-$K$ Candidates in Stage II}
    \label{tab:refinerag_topk_ablation}
    \begin{tabular}{c c c cc}
        \toprule
        \multirow{2}{*}{\textbf{Dataset}} &
        \multirow{2}{*}{\textbf{$K$}} &
        \multirow{2}{*}{\textbf{F1-score$\uparrow$}} &
        \multicolumn{2}{c}{\textbf{ASR$\uparrow$}} \\
        \cmidrule(lr){4-5}
        & & & \textbf{Llama} & \textbf{Vicuna} \\
        \midrule
        \multirow{3}{*}{\textbf{NQ}} 
            & 10 & 0.85 & 0.87 & \textbf{0.86} \\
            & 20 & \textbf{0.89} & \textbf{0.90} & 0.85 \\
            & 30 & \textbf{0.89} & 0.87 & 0.85 \\
        \midrule
        \multirow{3}{*}{\textbf{MSMARCO}} 
            & 10 & 0.67 & 0.80 & 0.80 \\
            & 20 & 0.70 & \textbf{0.83} & \textbf{0.81} \\
            & 30 & \textbf{0.72} & 0.82 & 0.77 \\
        \bottomrule
    \end{tabular}
\end{table}
